Beam test measurements of Low Gain Avalanche Detector single pads and arrays for the ATLAS High Granularity Timing Detector

For the high luminosity upgrade of the LHC at CERN, ATLAS is considering the addition of a High Granularity Timing Detector (HGTD) in front of the end cap and forward calorimeters at |z| = 3.5 m and covering the region 2.4 < |{\eta}| < 4 to help reducing the effect of pile-up. The chosen sensors are arrays of 50 {\mu}m thin Low Gain Avalanche Detectors (LGAD). This paper presents results on single LGAD sensors with a surface area of 1.3x1.3 mm2 and arrays with 2x2 pads with a surface area of 2x2 mm^2 or 3x3 mm^2 each and different implant doses of the p+ multiplication layer. They are obtained from data collected during a beam test campaign in Autumn 2016 with a pion beam of 120 GeV energy at the CERN SPS. In addition to several quantities measured inclusively for each pad, the gain, efficiency and time resolution have been estimated as a function of the position of the incident particle inside the pad by using a beam telescope with a position resolution of few {\mu}m. Different methods to measure the time resolution are compared, yielding consistent results. The sensors with a surface area of 1.3x1.3 mm^2 have a time resolution of about 40 ps for a gain of 20 and of about 27 ps for a gain of 50 and fulfill the HGTD requirements. Larger sensors have, as expected, a degraded time resolution. All sensors show very good efficiency and time resolution uniformity.

==> Makefile <==
# Makefile for creating an ATLAS paper draft using journal classes

TEXLIVE  = 2016
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = bibtex
DVIPS    = dvips
DVIPDF   = dvipdf
OPEN     = open

TEXFILES = $(wildcard *.tex)

.PHONY: texlive clean

all: atlas-jinst

texlive:
	for file in $(TEXFILES); do \
	  if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	    echo "Changing texlive value in $$file"; \
	    sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $$file; \
	  else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \
	done

atlas-elsevier: atlas-elsevier.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-jhep: atlas-jhep.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-jinst: atlas-jinst.pdf
	@echo "Made $<"
	$(OPEN) $<

atlas-revtex: atlas-revtex.pdf
	@echo "Made $<"
	# $(OPEN) $<

run_latex: $(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $< and $(basename $<).pdf"

# Standard LaTeX targets
%.pdf: %.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.dvi: $(BASENAME).tex
	$(LATEX)    $<
	$(LATEX)    $<

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf \
	 *.spl *-revtexNotes.bib *.run.xml *.synctex.gz *~

cleanall: clean
	-rm *.pdf


==> acknowledgements/Acknowledgements.tex <==
% Acknowledgements for papers with collision data
% Version 18-Jan-2017

% Standard acknowledgements start here
%----------------------------------------------
We thank CERN for the very successful operation of the LHC, as well as the
support staff from our institutions without whom ATLAS could not be
operated efficiently.

We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC, Australia; BMWFW and FWF, Austria; ANAS, Azerbaijan; SSTC, Belarus; CNPq and FAPESP, Brazil; NSERC, NRC and CFI, Canada; CERN; CONICYT, Chile; CAS, MOST and NSFC, China; COLCIENCIAS, Colombia; MSMT CR, MPO CR and VSC CR, Czech Republic; DNRF and DNSRC, Denmark; IN2P3-CNRS, CEA-DSM/IRFU, France; GNSF, Georgia; BMBF, HGF, and MPG, Germany; GSRT, Greece; RGC, Hong Kong SAR, China; ISF, I-CORE and Benoziyo Center, Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco; FOM and NWO, Netherlands; RCN, Norway; MNiSW and NCN, Poland; FCT, Portugal; MNE/IFA, Romania; MES of Russia and NRC KI, Russian Federation; JINR; MESTD, Serbia; MSSR, Slovakia; ARRS and MIZ\v{S}, Slovenia; DST/NRF, South Africa; MINECO, Spain; SRC and Wallenberg Foundation, Sweden; SERI, SNSF and Cantons of Bern and Geneva, Switzerland; MOST, Taiwan; TAEK, Turkey; STFC, United Kingdom; DOE and NSF, United States of America. In addition, individual groups and members have received support from BCKDF, the Canada Council, CANARIE, CRC, Compute Canada, FQRNT, and the Ontario Innovation Trust, Canada; EPLANET, ERC, ERDF, FP7, Horizon 2020 and Marie Sk{\l}odowska-Curie Actions, European Union; Investissements d'Avenir Labex and Idex, ANR, R{\'e}gion Auvergne and Fondation Partager le Savoir, France; DFG and AvH Foundation, Germany; Herakleitos, Thales and Aristeia programmes co-financed by EU-ESF and the Greek NSRF; BSF, GIF and Minerva, Israel; BRF, Norway; CERCA Programme Generalitat de Catalunya, Generalitat Valenciana, Spain; the Royal Society and Leverhulme Trust, United Kingdom.

The crucial computing support from all WLCG partners is acknowledged gratefully, in particular from CERN, the ATLAS Tier-1 facilities at TRIUMF (Canada), NDGF (Denmark, Norway, Sweden), CC-IN2P3 (France), KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain), ASGC (Taiwan), RAL (UK) and BNL (USA), the Tier-2 facilities worldwide and large non-WLCG resource providers. Major contributors of computing resources are listed in Ref.~\cite{ATL-GEN-PUB-2016-002}.
%----------------------------------------------



==> acknowledgements/Makefile <==
# Makefile for creating ATLAS Acknowledegments

TEXLIVE  = 2016
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = biber
DVIPS    = dvips
DVIPDF   = dvipdf

BASENAME = Acknowledgements-main

.PHONY: clean cleanpdf

run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Change TeX Live version
texlive: $(BASENAME).tex
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  echo "Changing texlive value in $$file"; \
	  sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $<; \
	else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \

# Standard LaTeX targets
$(BASENAME).pdf: $(BASENAME).tex
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.bbl: %.tex *.bib
	$(PDFLATEX) $*
	$(BIBTEX) $*

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf *-blx.bib \
	 *.run.xml *.synctex.gz *~

cleanpdf:
	-rm $(BASENAME).pdf

cleanall: clean cleanpdf


==> text/Todo.tex <==
\subsection*{2.2}
\begin{itemize}
\item More details for UCSC board
\item Comments by Laurent:\\ 
Line 165: Ref. 3 do not contain much more details...... Can we add a simple electrical schematic ? There is no comment on how the bias voltage is connected ?
\item Less detailed description of IN2P3 readout board
\end{itemize}

\subsection*{2.3}
\begin{itemize}
\item Add information on large SiPM
\end{itemize}

\subsection*{4.1}
\begin{itemize}
\item Comments by Laurent:\\ 
Line 276: Laser signal and MIP do not have the same signal shape so would have a different gain but this is not due to the trans-impedance uncertainty. Should/could the uncertainty be reduced?
\end{itemize}

\subsection*{5.2}
\begin{itemize}
\item Comments by Laurent:\\
Fig 15: I would prefer to remove two these plots and a zoom around the interpads region.\\ 
How the 40 mum error is estimated ?
\end{itemize}

\subsection*{5.3}
\begin{itemize}
\item Fix style of Figures, clarify what the two puls shapes are\\
\item Check what is done in the efficiency plots for events with crosstalk hits\\
\end{itemize}

\subsection*{Acknowledgements}
\begin{itemize}
\item Check that all relevant funding agencies are mentioned
\end{itemize}

